Towards Understanding Emotions in Informal Developer Interactions: A Gitter Chat Study

Emotions play a significant role in teamwork and collaborative activities like software development. While researchers have analyzed developer emotions in various software artifacts (e.g., issues, pull requests), few studies have focused on understanding the broad spectrum of emotions expressed in chats. As one of the most widely used means of communication, chats contain valuable information in the form of informal conversations, such as negative perspectives about adopting a tool. In this paper, we present a dataset of developer chat messages manually annotated with a wide range of emotion labels (and sub-labels), and analyze the type of information present in those messages. We also investigate the unique signals of emotions specific to chats and distinguish them from other forms of software communication. Our findings suggest that chats have fewer expressions of Approval and Fear but more expressions of Curiosity compared to GitHub comments. We also notice that Confusion is frequently observed when discussing programming-related information such as unexpected software behavior. Overall, our study highlights the potential of mining emotions in developer chats for supporting software maintenance and evolution tools.

==> Background.tex <==
\section{Background and Related Work}
\label{background}


\begin{table}
\centering
\small
\caption{Shaver's~\cite{Shaver} tree-structured emotion categories \newline (additional categories from GoEmotions~\cite{goemotions} shown in blue)}
\begin{tabular} { | p{1cm} | p{1.4cm} | p{4.8cm} | }
\hline
    Basic Emotion & Secondary Emotion & Tertiary Emotion \\ \hline\hline
    
     & Irritation & Annoyance, Agitation, Grumpiness, Aggravation, Grouchiness \\ \cline{2-3}
     & Exasperation & Frustration \\ \cline{2-3}
     & Rage & Anger, Fury, Hate, Dislike, Resentment, Outrage, Wrath, Hostility, Bitterness, Ferocity, Loathing, Scorn, Spite, Vengefulness \\ \cline{2-3}
     Anger & Envy & Jealousy \\ \cline{2-3}
     & Disgust & Revulsion, Contempt, Loathing \\  \cline{2-3}
     & Torment & - \\ \cline{2-3}
     & \textcolor{blue}{Disapproval} & - \\ \hline
     \hline

     & Affection  & Liking, Caring, Compassion, Fondness, Affection, Love, Attraction, Tenderness, Sentimentality, Adoration \\ \cline{2-3}
    Love & Lust & Desire, Passion, Infatuation \\ \cline{2-3}
     & Longing  & - \\ \hline
    \hline
    & Horror & Alarm, Fright, Panic, Terror, Fear, Hysteria, Shock, Mortification \\ \cline{2-3}
    Fear & Nervousness & Anxiety, Distress, Worry, Uneasiness, Tenseness, Apprehension, Dread \\ \hline
    \hline
     & Cheerfulness & Happiness, Amusement, Satisfaction, Bliss, Gaiety, Glee, Jolliness, Joviality, Joy, Delight, Enjoyment, Gladness, Jubilation, Elation, Ecstasy, Euphoria \\ \cline{2-3}
     & Zest & Enthusiasm, Excitement, Thrill, Zeal, Exhilaration \\ \cline{2-3}
     & Contentment & Pleasure \\ \cline{2-3}
     & Optimism & Eagerness, Hope \\  \cline{2-3}
     Joy & Pride & Triumph \\ \cline{2-3}
     & Enthrallment & Enthrallment, Rapture \\ \cline{2-3}
     & Relief & - \\ \cline{2-3}
     & \textcolor{blue}{Approval} & - \\ \cline{2-3}
     & \textcolor{blue}{Admiration} & - \\ \cline{2-3}
     \hline
    \hline
    & Suffering & Hurt, Anguish, Agony \\ \cline{2-3}
    & Sadness & Depression, Sorrow, Despair, Gloom, Hopelessness, Glumness, Unhappiness, Grief, Woe, Misery, Melancholy \\ \cline{2-3}
    & Disappoint & Displeasure, Dismay \\ \cline{2-3}
    Sadness & Shame & Guilt, Regret, Remorse \\ \cline{2-3}
    & Neglect & Embarrassment, Insecurity, Insult, Rejection, Alienation, Isolation, Loneliness, Homesickness, Defeat, Dejection, Humiliation \\ \cline{2-3}
    & Sympathy & Pity \\ \hline 
    \hline
    & Surprise & Amazement, Astonishment \\ \cline{2-3}
    & \textcolor{blue}{Confusion} & -  \\ \cline{2-3}
    Surprise & \textcolor{blue}{Curiosity} & -  \\ \cline{2-3}
    & \textcolor{blue}{Realization} & - \\ \hline 
\end{tabular}
\label{tab:shavers_category}
\end{table}

\textbf{Emotion Taxonomies.}
%add VAD and possibly revise the last paragraph.
\textcolor{blue}{ Performing emotion recognition naturally requires a clear definition of what emotions exist. Researchers often rely on psychological findings to determine the emotion categories they will use to further their studies. The field of psychology, however, does not offer a single agreed-upon taxonomy of human emotions. Although emotions have been studied for a long time, researchers have yet to reach a consensus on a taxonomy for human emotions \cite{zad2021emotion}. As a result, pursuing a better understanding of our emotions has led to the creation of various systems for categorizing emotions.
}
%Lastly, it's worth noting that although emotions have been studied for a long time, there is no final consensus on the taxonomy of human emotions \cite{zad2021emotion}. Pursuing a better understanding of our emotions has led to the creation of various systems for emotion categorization.
% By leveraging psychological studies, researchers have used several categorizations to detect emotions in written text. For instance,


\textcolor{blue}{
Among the most well-known proposed taxonomies for emotions is the Plutchik's model ~\cite{plutchik1980general}. This model represents the emotions as a wheel-like structure with three concentric circles (layers) of emotions and eight basic emotion categories: anger, disgust, fear, joy, sadness, surprise, trust, and anticipation. 
}
%The wheel of emotions is represented as concentric circles with the innermost representing pure, intense emotions and outer circles representing less intense or combined emotions.
%Plutchik's wheel of emotions is the model in psychology that uses these eight categories, their intensities, and the ways in which they interact with one another to interpret our emotions. The concept of the wheel pictures a number of concentric circles, each containing a variation of the eight mentioned emotion categories. The innermost circle represents the eight emotions in their purest, most intense form. By gradually moving toward the outermost circle, the emotions become less and less intense, while some are combined with each other to create new emotions \cite{plutchik1980general}. 
% there are other taxonomies 
%Other than Plutchik's, there are a few other well-known emotion taxonomies. 
%we can mention Ekman's taxonomy as one of the more well-known taxonomies, which presents six out of the eight abovementioned categories (i.e., anger, disgust, fear, happiness, sadness, and surprise) as the basic human emotions.
\textcolor{blue}{
Another widely recognized model of emotions is the work of Ekman et al.~\cite{Ekman1999}, who categorized emotions into six basic categories:  anger, disgust, fear, joy, sadness, and surprise. In a different study, Shaver et al.~\cite{Shaver} identified six basic emotion categories: love, joy, anger, sadness, surprise, and fear. According to Shaver et al., these basic emotions can be expanded in a treelike structure that allows the model to accommodate other emotions as subcategories.
In a more recent study, Parrot et al. further refined and developed Shaver's taxonomy and introduced a hierarchy with secondary and tertiary levels of emotions \cite{parrott2001emotions}. For instance, Parrot et al.'s taxonomy recognizes disappointment and sympathy as second-level emotions and subcategories of sadness, while displeasure and dismay are third-level emotions and subcategories of disappointment. \textcolor{red}{This need a table like Imran's to show categories} Additionally, in three different works, Cowen et al. have tried identifying various forms of human emotions using a combination of short videos and self-reports \cite{cowen2017self}, human vocalizations \cite{cowen2019mapping}, and facial expressions \cite{cowen2020face}. These efforts resulted in the identification of 27, 24, and 28 emotion categories, respectively.
}

\textcolor{blue}{Dimensional models of affect, on the other hand, have a different approach to understanding emotions. In order to better conceptualize the complexities of human emotions, these models represent various states of human emotions as a mixture of multiple qualities e.g., excitement and stress \cite{posner2005circumplex}. A simplified bi-dimensional variant of these models, commonly known as VAD \cite{russell1977evidence}, has been used to categorize emotions into the four categories of stress, excitement, depression, and relaxation \cite{deva}.
}

\textcolor{blue}{
Although a universally accepted taxonomy of emotions does not exist, it is widely accepted that emotions are made up of basic categories combined to form more elaborate emotions \cite{sanei2021impacts}. This study uses a combination of Plutchik's, Ekman's, and Parrots's taxonomies, as well as the VAD model's emotion categories to assess the performance of each emotion recognition tool with respect to the categories recognized by the tool.
}

% Despite being studied for a long time, there is no consensus on the taxonomy of human emotions \cite{zad2021emotion}. Pursuing a better understanding of our emotions has led to the creation of various systems for emotion categorization. Ekman's is among the well-known emotion taxonomies that presents six categories (i.e., anger, disgust, fear, happiness, sadness, and surprise) as basic human emotions \cite{ekman2011meant}. Another example, Shaver's taxonomy, classifies emotions into categories of love, joy, anger, sadness, fear, and surprise \cite{shaver1987emotion}. Further, a taxonomy by Plutchik, also known as the wheel of emotions, proposes a model that categorizes emotions into eight basic categories of anger, trust, fear, disgust, surprise, joy, sadness, and anticipation which can be combined with one another to create more complex emotions or based on the level of their intensity, be experienced in a further purified state \cite{plutchik1980general}. There is often intricate psychological bases for these taxonomies, which pushes examining their details beyond the scope of the present paper. For this study, we rely on Plutchik's emotion taxonomy  for basic emotions to analyze the developers' communications by performing emotion analysis.
 

% There are a number of tools available for both sentiment and emotion analysis. Some sentiment analysis tools include:
% \begin{itemize}
%     \item General: VADER, Stanford CoreNLP, SentiStrength, NLTK
%     \item SE-specific: SentiStrength-SE, SentiCR, Senti4SD
% \end{itemize}
% And some emotion analysis tools are:
% \begin{itemize}
%     \item General: VADER, Stanford CoreNLP, SentiStrength, NLTK
%     \item SE-specific: SentiStrength-SE, SentiCR, Senti4SD
% \end{itemize}


% what is emotion - Wheel of emotions
%Emotions are the means through which the feelings of individuals or groups are described \cite{zad2021emotion}. The eight basic human emotions include joy, fear, surprise, trust, and their counterparts: sadness, anger, anticipation, and disgust. 

\vspace{0.1cm}
\noindent
\textbf{Emotion Analysis in SE.}
Previous research shows that emotion is prevalent in software engineering (SE) teams, and that developers experience a wide range of emotions during collaborative tasks. Specific emotions such as anger, joy, and fear, were identified in GitHub~\cite{emod}.% comments \cite{emod}, and issue reports \cite{p132}. %\cite{esem-e, p31, p131}
%\cite{p44} %Researchers have also detected other emotions such as confusion in code reviews \cite{Ebert2021AnES}. 
More recently, researchers studied toxicity in issue reports~\cite{miller2022did}, and confusion in code reviews~\cite{Ebert2021AnES}.%, and politeness in bug reports~\cite{p31}. %\cite{p130, p131}
%Affective trust between developers in a project was also found in pull request or commit comments~\cite{Sajadi2023, p149, arsenalgsd, calefato2016affective}.
To the best of our knowledge, this is the first study to analyze developer emotions in Gitter chat communications.


% reasons Plutchik's taxonomy is the best
% any emotion detection/analysis relies on a taxonomy
%As empathetic creatures, human beings put a heavy emphasis on their perceived emotions, which makes the identification and understanding of emotions all the more valuable \cite{felbermayr2016role}. 
%Many attempts have been made to automate the task of emotion detection, 
%and naturally, all have required a predetermined set of emotion categories \cite{zad2021emotion}. This need for a clear taxonomy of emotions in related studies is often answered by reliance on psychological studies attempting to provide said categories \cite{venigalla2021understanding, murgia2014developers, calefato2019emtk, neupane2019emod, destefanis2018measuring, murgia2018exploratory}.
% Built upon psychological bases, the wheel of emotions or Plutchik's emotion taxonomy is a tried and tested model that provides us with these emotion categories.

% Related work
% Several ML-based techniques have been proposed to automatically detect emotion in software-related text~\cite{esem-e, emtk, ortu2016}. 
%Murgia et al. proposed an approach~\cite{esem-e} to detect three basic emotions in a JIRA dataset~\cite{ortu2016}. More recently, Calefato et al. developed a machine learning-based technique EMTk~\cite{emtk} to identify six primary emotions according to Shaver’s framework~\cite{Shaver}, and was evaluated on a StackOverflow dataset~\cite{novielli2018gold}. 
%Neupane et al.~\cite{emod} investigated emotion dynamics in GitHub repositories, using EMTk as their primary model. Cabrera-Diego et al.~\cite{cabrera2020classifying} used the multi-label classifiers HOMER~\cite{tsoumakas2008effective} and RAkEL~\cite{tsoumakas2010random} and found these tools to be more effective than EMTK. 
Furthermore, emotion detection using lexicon-based approaches in SE have been scarce.
Lexicons such as LIWC \cite{liwc}, WordNet Affect \cite{wordnetaffect}, and NRC \cite{mohammad2013nrc} have been used to detect emotions with high levels of accuracy for general purpose text~\cite{8798675}. 
%Most of these available tools are, however, developed to work with general text and are not necessarily apt for use cases within the software development context. Nevertheless, there have been attempts to leverage such tools for analyzing software-related text \cite{licorish2021relating, venigalla2021understanding}.
% While Natural Language Processing has been achieving new feats in the field, lexicon-based approaches and tools such as LIWC are widely used to detect emotions and
\textcolor{blue}{With regard to software engineering text,} Venigalla et al. analyzed software developers' emotions towards software documentation using the NRC lexicon~\cite{venigalla2021understanding}. \textcolor{blue}{Additionally, DEVA \cite{deva}, a tool using the VAD emotion model, also relies on a lexicon for detecting emotions.}
